ProFLingo: A Fingerprinting-based Intellectual Property Protection Scheme for Large Language Models

Large language models (LLMs) have attracted significant attention in recent years. Due to their "Large" nature, training LLMs from scratch consumes immense computational resources. Since several major players in the artificial intelligence (AI) field have open-sourced their original LLMs, an increasing number of individuals and smaller companies are able to build derivative LLMs based on these open-sourced models at much lower costs. However, this practice opens up possibilities for unauthorized use or reproduction that may not comply with licensing agreements, and fine-tuning can change the model's behavior, thus complicating the determination of model ownership. Current intellectual property (IP) protection schemes for LLMs are either designed for white-box settings or require additional modifications to the original model, which restricts their use in real-world settings. In this paper, we propose ProFLingo, a black-box fingerprinting-based IP protection scheme for LLMs. ProFLingo generates queries that elicit specific responses from an original model, thereby establishing unique fingerprints. Our scheme assesses the effectiveness of these queries on a suspect model to determine whether it has been derived from the original model. ProFLingo offers a non-invasive approach, which neither requires knowledge of the suspect model nor modifications to the base model or its training process. To the best of our knowledge, our method represents the first black-box fingerprinting technique for IP protection for LLMs. Our source code and generated queries are available at: https://github.com/hengvt/ProFLingo.

==> Discussion.tex <==
\section{Discussion}
\label{sec:discuss} 

\noindent \textbf{Why are ASRs for related models high?} \\ The nature of adversarial examples is widely acknowledged to represent the decision boundary of the model, which in turn reflects the distribution of the training data \cite{Tanay16:arXiv:ae}. It is therefore expected that two models with similar architectures, trained on the same dataset and using a similar training process, will develop sufficiently similar decision boundaries to allow the transfer of AEs. While this paper focuses on fine-tuning, the essence of \sysname is to analyze the decision boundary similarities between two models, with the ASR serving as an indicator of the connection or relationship between them. Nonetheless, achieving similar decision boundaries between two LLMs is more difficult than it does with traditional models, mainly due to the complexity and capacity of LLMs, and the high ASRs of same-family models do not undermine the effectiveness of \sysname, as it remains impractical for external entities to independently train a model from scratch to achieve such a high level of similarity.
\\ \\ 
\noindent \textbf{Is \sysname effective against model extraction?} \\
Base models may also be utilized for training new models from scratch by using their outputs, a practice referred to as model extraction, model stealing, or knowledge distillation when white-box access to the base model is available. Unfortunately, no existing IP protection schemes for LLMs, including both black-box and white-box approaches, can protect the base model against model extraction. While adversarial examples have shown resilience against model extraction in traditional image models, it is challenging for AEs in LLMs to exhibit similar resistance due to the complexity of LLMs' decision boundaries. Model extraction requires significantly more computational resources than fine-tuning, so we cannot perform model extraction by ourselves or find enough distilled models to conduct comprehensive experiments. However, when we tried to use \sysname verify MiniMA-3B \cite{Zhang23:arXiv:minima}, a model distilled from Llama-2-7b, our attacks resulted in a high ASR of 0.24. This result suggests that \sysname might offer a defense against model extraction. Still, additional research is required to confirm this capability.
\\ \\ 
\noindent \textbf{Is \sysname useful for watermarked models?} \\
Yes. While black-box watermarks, generally based on backdoor attacks, exhibit behavior that is similar to adversarial examples, where designed prompts are used as inputs to force the model to produce abnormal outputs, the underlying mechanisms differ. Black-box watermarking aims to embed a trigger in the model with the expectation that it will be retained after fine-tuning. In other words, black-box watermarking forces the model to ``remember" something. Conversely, Black-box fingerprinting finds inputs that barely cross the decision boundary, with the expectation that certain portions of the decision boundary will not significantly change after fine-tuning. Both techniques can be integrated into a comprehensive metric to determine if a suspect model is fine-tuned from an original model. The failure of one method does not imply the failure of the other. Additionally, the number of triggers that can be embedded is limited, and triggers are predetermined before the model's release. Once such triggers are exposed, the model can be fine-tuned to neutralize them deliberately. In contrast, although \sysname is also vulnerable to such deliberate fine-tuning, there are virtually infinite adversarial examples, and we can continually generate new ones to evaluate newly fine-tuned models even when old ones are exposed.

